Enhancing Dynamical System Modeling through Interpretable Machine Learning Augmentations: A Case Study in Cathodic Electrophoretic Deposition

We introduce a comprehensive data-driven framework aimed at enhancing the modeling of physical systems, employing inference techniques and machine learning enhancements. As a demonstrative application, we pursue the modeling of cathodic electrophoretic deposition (EPD), commonly known as e-coating. Our approach illustrates a systematic procedure for enhancing physical models by identifying their limitations through inference on experimental data and introducing adaptable model enhancements to address these shortcomings. We begin by tackling the issue of model parameter identifiability, which reveals aspects of the model that require improvement. To address generalizability , we introduce modifications which also enhance identifiability. However, these modifications do not fully capture essential experimental behaviors. To overcome this limitation, we incorporate interpretable yet flexible augmentations into the baseline model. These augmentations are parameterized by simple fully-connected neural networks (FNNs), and we leverage machine learning tools, particularly Neural Ordinary Differential Equations (Neural ODEs), to learn these augmentations. Our simulations demonstrate that the machine learning-augmented model more accurately captures observed behaviors and improves predictive accuracy. Nevertheless, we contend that while the model updates offer superior performance and capture the relevant physics, we can reduce off-line computational costs by eliminating certain dynamics without compromising accuracy or interpretability in downstream predictions of quantities of interest, particularly film thickness predictions. The entire process outlined here provides a structured approach to leverage data-driven methods. Firstly, it helps us comprehend the root causes of model inaccuracies, and secondly, it offers a principled method for enhancing model performance.

==> 4_ml_framework.tex <==
\section{Computational Framework}
\subsection{Computations}
\subsubsection{1D}

We consider the 1D problem with a domain of size $L$ where the cathode located is at x=0 and the anode is located at x=L. The 1D Poisson problem is solved only on this interval.

\begin{figure}[h!]
\centering
\tikzsetnextfilename{1Dsetup}
\begin{tikzpicture}[scale=5]
\tikzstyle{every node}=[font=\small]
\draw[line width=0.5pt] (0,0.0) -- (1,0.0); 
\draw[line width=2pt] (0.0,-0.1) -- (0.0,0.1); 
\draw[line width=2pt] (1.0,-0.1) -- (1.0,0.1); 

\node[draw=none,rotate=90] at (-0.1,0.0) {$\textrm{cathode}$};
\node[draw=none,rotate=90] at (1.1,0.0) {$\textrm{anode}$};
\node[draw=none] at (0,-0.15) {$x=0$};
\node[draw=none] at (1,-0.15) {$x=L$};
\fill[gray,opacity=0.3] (0.0,-0.1) rectangle (0.1,0.1);
\node[draw=none] at (0.2,0.2) {film};
\draw[-stealth,line width=0.5pt] (0.20,0.15) -- (0.05,0.15) -- (0.05,0.1); 
\end{tikzpicture}
\caption{Initial setup for the 1D case.\label{fig:1DSetup}}
\end{figure}

For the electric field, we solve a Poisson equation with Robin boundary condition on the interface bath/film.
%\begin{align}
%\sigma_{\rm{bath}}\frac{\partial^2\phi}{\partial x^2}&=0 &\textrm{ in the bath}\\
%\phi-R_{\textrm{film}} \sigma_{\rm{bath}}\frac{\partial \phi}{\partial x}&=0 &\textrm{ at the interface film-bath}\\
%\phi_{\rm{anode}}(t) &= \phi_{t=0}+0.1 t & \textrm{ at the anode}
%\end{align}

\begin{align}
\sigma_{\rm{bath}}\frac{\partial^2\phi}{\partial x^2}&=0 &\textrm{ in the bath}\\
\phi-R_{\textrm{film}} \sigma_{\rm{bath}}\frac{\partial \phi}{\partial x}&=0 &\textrm{ at the interface film-bath}\\
\phi_{\rm{anode}}(t) &= \phi_{t=0} + \phi_{\rm{ramp}}(t) & \textrm{ at the anode}
\end{align}

Regarding the evolution of the film thickness and the resistance of the film, we use a decoupled approach (during the last meeting, it was said to be solved in an implicit coupled way).

The onset condition implemented for this simulation is the minimum current with $j_{\min}$=1 $A/m^{2}$. The thickness of the film is updated using:
\begin{align}
h(t+\Delta t) = h(t) + \Delta t C j_n
\end{align}

The value of the $R_{\textrm{film}}$, the film resistance is updated
\begin{align}
R_{\textrm{film}}(t+\Delta t) &=R_{\textrm{film}}(t)+\Delta t \rho(\bm{j}) C j_n
\end{align}


Regarding the effect of the film on the computational domain, we can choose among the following options:
\begin{enumerate}
\item Keep the same length for the bath, meaning that the film has no thickness but is only a boundary condition for the electric field problem
\item Decrease the length of the bath and modify the stencil of the laplace operator and even remove elements as the film thickness increases
%\item sub-iterate within a time-step to accurately capture the physical properties (Laplace Robin BC $\leftrightarrow$ $R_{\textrm{film}}$)
\end{enumerate}


For the current simulation, the length of the bath is not modified. A summary of all the parameters used is given in Table \ref{table:paramSim}. The final time is $t_{\rm{final}}=300s$. The length of the bath is $L=1$ m. The electric potential is initially 0 at the anode.

The evolution in time of the electric potential is given is Fig. \ref{fig:ElectricPotentialTime}. At the early stage, since no film is deposited, the electric potential is 0 at x=0 (potential of the cathode). As the film is deposited, the electric potential at the interface of the film grows.

\setlength{\tabcolsep}{0.35em}
\begin{table}[h]
\begin{center}
\caption{Summary of the parameters provided by Ford.}
\begin{tabular}{lcclccccccc}
\hline
Name & symbol & value & unit\\
\hline
Bath conductivity & $\sigma_{\rm{bath}}$ & 0.14 &$S/m$\\
Volumetric Coulombic efficiency & $C_v$ & 2e-8 &$m^3/C$ \\
Mass Coulombic efficiency & $C_m$ & 2.8e-5 & $kg/C$\\
Dry film density & $\rho_{\rm{dry}}$& 1,400 & $kg/m^3$\\
Film resistivity & $\rho(\bm{j})$&$\max\left(8.10^6 e^{-0.1|\textbf{j}|}\,,\,2.10^6\right)$&$\Omega .m$\\
Minimum current & $j_{\min}$ & 1 & $A/m^2$\\
Minimum charge & $Q_{\min}$&150&$C/m^2$\\
Initial resistance at cathode& $R_0$ & 0.5 & $\Omega . m^2$\\
\hline
\end{tabular}
\label{table:paramSim}
\end{center}
\end{table}

{\color{red}Show results using parameters provided by Ford }
